Encoding Lean's Type Theory in Dedukti

The Lean proof assistant has a rich library of mathematical formalizations that are interesting to users of other proof assistants. To help with the translation of this library to other systems, we present a theory in the Dedukti logical framework in which one can encode Lean terms and types, and define a typability-preserving translation from some large subset of Lean to that Dedukti theory.

==> prf-sr.tex <==
\hide{
Moreover, replacing a level by an equivalent one does not change
typing:

\begin{theorem}\label{th-sr-simeq}
  \hide{
  Let $\leftrightarrow$ be the relation on Dedukti terms which
  replaces a subterm $|l|$ by $|l'|$ if $l\simeq l'$;
  $\G\leftrightarrow\G'$ iff there are $\G_1,x,A,A',s,\G_2$ such that
  $\G=\G_1,x:A,\G_2$, $\G'=\G_1,x:A',\G_2$ and $A\leftrightarrow A'$;
  $\sim$ be the reflexive-transitive closure of $\leftrightarrow$.
  }
  %
  In any PTS, the monotone closure of a relation $R$ preserves typing
  if $R$ preserves typing and ${R}\sle{\equiv}$.
  %
  \hide{
  For all relations $R\sle\equiv_D$ that preserves typing (if
  $\G\th_D t:A$ and $tRu$ then $\G\th_D u:A$), if $\G\th_D t\!:\!A$
  then 1) if $tC[R]u$ then $\G\th_D u\!:\!A$, 2) if $\G C[R]\G'$ then
  $\G'\th_D t:A$, where $C[R]$ is the closure by context of $R$.
  }
\end{theorem}

\begin{proof}
  Usual subject-reduction proof in dependent type theory (details in
  \cite{blanqui26ictac-long}).
\end{proof}
}

\begin{proof}
  We simultaneously prove that, if $\G\th t:A$ then (1) if $t\cM_\cR
  t'$ then $\G\th t':A$, and (2) if $\G\cC_\cR\G'$ then $\G'\th t:A$,
  by induction on $\G\th t:A$. If $t\cR t'$ then $\G\th t':A$ since,
  by assumption, $\cR$ preserves typing. Otherwise, the reduction
  takes place in a strict subterm of $t$. We then proceed by case on
  the last typing rule used to get $\G\th t:A$. We only detail a few
  cases; the other cases easily follow by induction hypothesis.
  \begin{itemize}
  \item (1) (app) $\cfrac{\G\th t:\Pi x\!:\!A,B\quad \G\th u:A}{\G\th
    tu:B[x/u]}$. There are two cases:
    \begin{itemize}
    \item $tu\cM_\cR t'u$ with $t\cM_\cR t'$. By
      induction hypothesis (1), $\G\th t':\Pi x\!:\!A,B$. Therefore,
      by (app), $\G\th t'u:B[x/u]$.
    \item $tu\cM_\cR tu'$ with $u\cM_\cR u'$. By induction hypothesis
      (1), $\G\th u':A$. By (app), $\G\th tu':B[x/u']$. By correctness
      of types, $\G\th\Pi x\!:\!A,B:s'\in\cS$. By inversion,
      $\G,x\!:\!A\th B:s\in\cS$. By substitution, $\G\th
      B[x/u]:s$. Since, by assumption, ${\cM_\cR}\sle{\equiv}$, we
      have $B[x/u']\equiv B[x/u]$. Therefore, by (conv), $\G\th
      tu':B[x/u]$.
    \end{itemize}
  \item (1) (lam) $\cfrac{\G,x\!:\!A\th t:B\quad \G\th\Pi
    x\!:\!A,B:s\in\cS}{\G\th \l x\!:\!A,t:\Pi x\!:\!A,B}$. There are
    two cases:
    \begin{itemize}
    \item $\l x\!:\!A,t\cM_\cR\l x\!:\!A',t$ with $A\cM_\cR A'$. By
      induction hypothesis, $\G,x\!:\!A'\th t:B$. By induction
      hypothesis, $\G\th\Pi x\!:\!A',B:s$. By (lam), $\G\th\l
      x\!:\!A',t:\Pi x\!:\!A',B$. Since, by assumption,
      ${\cM_\cR}\sle{\equiv}$, we have $\Pi x\!:\!A',B\equiv\Pi
      x\!:\!A,B$. Therefore, by (conv), $\G\th\l x\!:\!A',t:\Pi
      x\!:\!A,B$.
    \item $\l x\!:\!A,t\cM_\cR\l x\!:\!A,t'$ with $t\cM_\cR t'$. By
      induction hypothesis (1), $\G,x\!:\!A\th t':B$. Therefore, by
      (lam), $\G\th\l x\!:\!A,t':\Pi x\!:\!A,B$.
    \end{itemize}
  \item (2) (decl) $\cfrac{\th\G\quad \G\th A:s\in\cS\quad
    x\notin\G}{\th\G,x\!:\!A}$. There are two cases:
    \begin{itemize}
    \item ${\G,x\!:\!A}\,\cC_\cR\,{\G',x\!:\!A}$ with
      $\G\cC_\cR\G'$. By induction hypothesis (2), $\th\G'$ and
      $\G'\th A:s$. Therefore, by (decl), $\th\G',x\!:\!A$.
    \item ${\G,x\!:\!A}\,\cC_\cR\,{\G,x\!:\!A'}$ with $A\cM_\cR
      A'$. By induction hypothesis (1), $\G\th A':s$. Therefore, by
      (decl), $\th\G,x:A'$.
    \end{itemize}
  \item (2) (var) $\cfrac{\th\G\quad x\!:\!A\in\G}{\G\th x:A}$. By
    induction hypothesis (1), $\th\G'$. Since $x\!:\!A\in\G$, there
    are $\G_1$ and $\G_2$ such that $\G=\G_1,x:A,\G_2$. There are two
    cases:
    \begin{itemize}
    \item $\G'=\G_1',x\!:\!A,\G_2$ and $\G_1\cM_\cR\G_1'$, or
      $\G'=\G_1,x\!:\!A,\G_2'$ and $\G_2\cM_\cR\G_2'$. In both cases,
      $x\!:\!A\in\G'$ and, by (var), $\G'\th x:A$.
    \item $\G'=\G_1,x\!:\!A',\G_2$ and $A\cM_\cR A'$. By (var), $\G\th
      x:A'$ and, by (conv), $\G\th x:A$.
    \end{itemize}
  \end{itemize}
\end{proof}

%%% Local Variables:
%%%   TeX-master: "main"
%%%   mode: LaTeX
%%%   ispell-local-dictionary: "english"
%%% End:

